Invocation-driven Neural Approximate Computing with a Multiclass-Classifier and Multiple Approximators

Neural approximate computing gains enormous energy-efficiency at the cost of tolerable quality-loss. A neural approximator can map the input data to output while a classifier determines whether the input data are safe to approximate with quality guarantee. However, existing works cannot maximize the invocation of the approximator, resulting in limited speedup and energy saving. By exploring the mapping space of those target functions, in this paper, we observe a nonuniform distribution of the approximation error incurred by the same approximator. We thus propose a novel approximate computing architecture with a Multiclass-Classifier and Multiple Approximators (MCMA). These approximators have identical network topologies and thus can share the same hardware resource in a neural processing unit(NPU) clip. In the runtime, MCMA can swap in the invoked approximator by merely shipping the synapse weights from the on-chip memory to the buffers near MAC within a cycle. We also propose efficient co-training methods for such MCMA architecture. Experimental results show a more substantial invocation of MCMA as well as the gain of energy-efficiency.

==> tex/architecture.tex <==
\section{FPGA Implementation}\label{sect:implement}

This work is built upon an off-the-shelf programable SoCs containing a PFGA. %Proposed architecture can integrate the main CPU and the programmable logic. 
The programmable logic resources accommodate the classifier-approximator architecture~(ACA) and the CPU~(ARM core) performs the accurate computation and control the data-path. The overall architecture is shown in Fig.~\ref{fig:dataflow}. Besides CPU, the accurate computation also needs memory and control unit. %CPU can control the overall data flow, and it can perform the accurate computing as well. 
The right part of the figure shows ACA, which is composed of BRAM memory, reconfigurable logic and DSPs for implementing NN models in the MAC and MCMA architecture. A multiplexer (MUX) is used to distribute the data samples to the approximator assigned by the multi-class classifier. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{images/chapter4/dataflow.pdf}\vspace{-10pt}
  \caption{Data-path for the ACA architecture.}
  \label{fig:dataflow}\vspace{-15pt}
\end{figure}

%\subsection{Architecture overview}
%The integrated architecture are composed of approximate parts and accurate computing part. 


%\subsection{Design Data Flow}

Fig.~\ref{fig:dataflow} also shows the data flow of the proposed architecture. The high throughput ARM Accelerator Coherency Port (ACP) is used to connect CPU part and ACA. In order to hide their communication latency, we implement the ACA in pipeline. In the initial step (step 1), CPU fetches the inputs into memory (one data batch at a time). Then, inputs are sent to ACA and stored in the BRAM memory in step 2. In step 3, data are fed into a multi-class classifier which can classify the inputs for approximate computing in proper accelerator or for accurate computing in CPU. The multi-class classifier generate a Mask code for each input sample to indicate the approximators through the multiplexers as shown in step 4. If the first bit of the mask is 1, it means the input data should be computed accurately. In this way, indices of input samples are extracted, %. A batch of such indices are then 
grouped and compressed. If the first bit of mask is 0, the selected approximator generates the results using input sample in step 5. Then, the partial results and compressed indices are sent back to memory in step 6. Those data that need accurate computation are directly fetched by CPU based on the indices in step 7. In the last step, CPU sends the computation result to memory and merge it with other results. Batches of input samples are fed into the data-path like a pipeline, in order to hide the latency of communication between CPU and ACA. 

The MCMA architecture is implemented either in ARM Cortex-a53~(v8) CPU as pure software, or in the FPGA as synthesized logic. The multilayer perceptron (MLP) models are used as the NN model for the multi-class classifier and the approximater; they are optimized using data-level parallelism and computation resources sharing~\cite{Wei-dac17}. In each layer of neurons, the input data are shared among the computing engines, while the weights are circled into the computing engines to mimic the synapses~(and neurons) in different layers. The weights are stored in the LUT where is close to DSP. All the neurons are fully unrolled and pipelined, so that all layers can be executed in parallel. 

The micriarchitecture of the proposed ACA architecture and the control of the data-path can be easily generated by high-level synthesis tool using our programming template.




==> tex/thebibliography.tex <==
\begin{thebibliography}{10}\scriptsize

\bibitem{baek2010green}
W.~Baek and T.~Chilimbi.
\newblock Green: a framework for supporting energy-conscious programming using
  controlled approximation.
\newblock In {\em Sigplan Notices}, pages 198--209, 2010.

\bibitem{du2014leveraging}
Z.~Du et al.
\newblock Leveraging the error resilience of machine-learning applications for
  designing highly energy efficient accelerators.
\newblock In {\em Asia and South Pacific Design Automation Conference}, pages 201--206, 2014.

\bibitem{esmaeilzadeh2012neural}
H.~Esmaeilzadeh et al.
\newblock Neural acceleration for general-purpose approximate programs.
\newblock In {\em International Symposium on Microarchitecture}, pages 449--460, 2012.

\bibitem{han2013approximate}
J.~Han and M.~Orshansky.
\newblock Approximate computing: An emerging paradigm for energy-efficient design.
\newblock In {\em European Test Symposium}, pages 1--6, 2013.

\bibitem{Imani-date16}
M.~Imani, A.~Rahimi, and T.~Rosing.
\newblock Resistive configurable associative memory for approximate computing.
\newblock In {\em Design, Automation Test in Europe Conference Exhibition}, pages 1327--1332, 2016.

\bibitem{khudia2015rumba}
D.~Khudia et al.
\newblock Rumba: an online quality management system for approximate computing.
\newblock In {\em SIGARCH Computer Architecture News}, pages 554--566, 2015.

\bibitem{Kim-dac16}
Y.~Kim et al.
\newblock Designing approximate circuits using clock overgating.
\newblock In {\em Design Automation Conference}, pages 1--6, 2016.

\bibitem{Liang-tc13}
J.~Liang, J.~Han, and F.~Lombardi.
\newblock New metrics for the reliability of approximate and probabilistic
  adders.
\newblock {\em Transactions on Computers}, pages 1760--1771, 2013.

\bibitem{mahajantowards}
D.~Mahajan et al.
\newblock Towards statistical guarantees in controlling quality tradeoffs for
  approximate acceleration.

\bibitem{Mohapatra-date11}
D.~Mohapatra et al.
\newblock Design of voltage-scalable meta-functions for approximate computing.
\newblock In {\em Design, Automation Test in Europe}, pages 1--6, 2011.

\bibitem{samadi2013sage}
M.~Samadi et al.
\newblock Sage: Self-tuning approximation for graphics engines.
\newblock In {\em International Symposium on Microarchitecture}, pages 13--24, 2013.

\bibitem{venkataramani2013quality}
S.~Venkataramani et al.
\newblock Quality programmable vector processors for approximate computing.
\newblock In {\em International Symposium on Microarchitecture}, pages 1--12, 2013.

\bibitem{wang2016effective}
T.~Wang et al.
\newblock On effective and efficient quality management for approximate
  computing.
\newblock In {\em International Symposium on Low Power Electronics and Design}, pages 156--161, 2016.

%new added
\bibitem{alawad2016}
M Alawad et al.
\newblock Survey of Stochastic-Based computation Paradigms.
\newblock In{\em},page.

%\bibitem{ye-iccad13}
%R.~Ye et al.
%\newblock On reconfiguration-oriented approximate adder design and its
%  application.
%\newblock In {\em International Conference on Computer-Aided Design}, pages 48--54, 2013.

\bibitem{Han2015Learning}
S.~Han et al.
\newblock Learning both Weights and Connections for Efficient Neural Networks.
\newblock In {\em Computer Science} , 2015.

\end{thebibliography}

